Low-Complexity Detection of M-ary PSK Faster-than-Nyquist Signaling

Faster-than-Nyquist (FTN) signaling is a promising non-orthogonal physical layer transmission technique to improve the spectral efficiency of future communication systems but at the expense of intersymbol-interference (ISI). In this paper, we investigate the detection problem of FTN signaling and formulate the sequence estimation problem of any $M$-ary phase shift keying (PSK) FTN signaling as an optimization problem that turns out to be non-convex and nondeterministic polynomial time (NP)-hard to solve. We propose a novel algorithm, based on concepts from semidefinite relaxation (SDR) and Gaussian randomization, to detect any $M$-ary PSK FTN signaling in polynomial time complexity regardless of the constellation size $M$ or the ISI length. Simulation results show that the proposed algorithm strikes a balance between the achieved performance and the computational complexity. Additionally, results show the merits of the proposed algorithm in improving the spectral efficiency when compared to Nyquist signaling and the state-of-the-art schemes from the literature. In particular, when compared to Nyquist signaling at the same error rate and signal-to-noise ratio, our scheme provides around $17\%$ increase in the spectral efficiency at a roll-off factor of 0.3.

==> formu_2.tex <==
\section{Proposed STSDRSE Technique} \label{sec:SDP2}

%\subsection{First Approach}
%The constraints in \eqref{eq:opML} is equivalent to 
%\begin{eqnarray}
%(a_n - 1)(a_n + 1)(a_n - 3)(a_n + 3) = 0, \quad n = 1, ..., 2N.
%\end{eqnarray}
%By introducing the auxiliary variables $b_n = a_n^2, n = 1, ..., 2N$, the constraints in  \eqref{eq:opML} can be further written as
%\begin{eqnarray}
%a_n^2 - b_n = 0, \quad n = 1, ..., 2N, \label{eq:const_1_n}\\
%b_n^2 - 10 b_n + 9 = 0, \quad n = 1, ..., 2N. \label{eq:const_2_n}
%\end{eqnarray}
%Let us formulate the optimization problem in \eqref{eq:opML} in higher dimension by defining 
%\begin{eqnarray}
%\bm{\omega}^{\rm{T}} &=& [\bm{a}^{\rm{T}} \: \bm{b}^{\rm{T}} \: 1], \\
%\bm{\Omega} &=& \bm{\omega} \: \bm{\omega}^{\rm{T}} = \begin{bmatrix}
%\bm{a} \bm{a}^{\rm{T}} & \bm{a} \bm{b}^{\rm{T}} & \bm{a}\\ 
%\bm{b} \bm{a}^{\rm{T}} & \bm{b} \bm{b}^{\rm{T}} & \bm{b}\\
%\bm{a}^{\rm{T}}        & \bm{b}^{\rm{T}}        & 1
%\end{bmatrix}.
%\end{eqnarray}
%Let us denote $\bm{\Omega}_{1,1} = \bm{a} \bm{a}^{\rm{T}}$, $\bm{\Omega}_{2,2} = \bm{b} \bm{b}^{\rm{T}}$, $\bm{\Omega}_{1,3} = \bm{a}$, and $\bm{\Omega}_{2,3} = \bm{b}$, where $\bm{\Omega}_{i,j}, i,j = 1, 2, 3,$ are the $(i,j)$th sub-blocks of $\bm{\Omega}$ of appropriate sizes. Hence, the constraints in \eqref{eq:const_1_n} and \eqref{eq:const_2_n} can be rewritten as
%\begin{eqnarray}
%\diag\{\bm{\Omega}_{1,1}\} - \bm{\Omega}_{2,3} = 0, \\
%\diag\{\bm{\Omega}_{2,2}\} - 10 \bm{\Omega}_{2,3} + 9 . \bm{1} = 0, \\
%\bm{\Omega}_{3,3} = 1, \\
%\bm{\Omega} \succeq 0, \\
%\rank\{\bm{\Omega}\} = 1.
%\end{eqnarray}
%
%The objective function in \eqref{eq:opML} can be rewritten in terms of $\bm{\Omega}$ as 
%\begin{eqnarray}
%\bm{\omega}^{\rm{T}} \: \bm{\Phi} \: \bm{\omega} = \Tr\{\bm{\Phi} \: \bm{\omega} \: \bm{\omega}^{\rm{T}}\} = \Tr\{\bm{\Phi} \: \bm{\Omega}\},
%\end{eqnarray}
%where 
%\begin{eqnarray}
%\bm{\Phi} = \begin{bmatrix}
%\bm{G} & \bm{0} & -\bm{y}\\ 
%\bm{0} & \bm{0} & \bm{0}\\
%- \bm{y}^{\rm{T}}        & \bm{0}        & \bm{z}^{\rm{T}} \bm{G} \bm{z}
%\end{bmatrix}
%\end{eqnarray}
%
%Finally, the optimization problem in \eqref{eq:opML} is expressed as
%\begin{eqnarray}
%\mathcal{OP}1: \qquad \underset{\bm{\Omega}}{\min} &\quad&  \Tr\{\bm{\Phi} \: \bm{\Omega}\}   \\
%{\textup{s. t.}} &\quad& \diag\{\bm{\Omega}_{1,1}\} - \bm{\Omega}_{2,3} = 0, \\
%&\quad& \diag\{\bm{\Omega}_{2,2}\} - 10 \bm{\Omega}_{2,3} + 9 . \bm{1} = 0, \\
%&\quad& \bm{\Omega}_{3,3} = 1, \\
%&\quad& \bm{\Omega} \succeq 0, \\
%&\quad& \rank\{\bm{\Omega}\} = 1. \label{eq:rank1}
%\end{eqnarray}
%
%The optimization problem $\mathcal{OP}1$ is non-convex due to the rank-one constraint in \eqref{eq:rank1}. By dropping this constraint, we reach the SDR of $\mathcal{OP}1$ 
%\begin{eqnarray}
%\mathcal{SDR}1: \qquad \underset{\bm{\Omega}}{\min} &\quad&  \Tr\{\bm{\Phi} \: \bm{\Omega}\}   \\
%{\textup{s. t.}} &\quad& \diag\{\bm{\Omega}_{1,1}\} - \bm{\Omega}_{2,3} = 0, \\
%&\quad& \diag\{\bm{\Omega}_{2,2}\} - 10 \bm{\Omega}_{2,3} + 9 . \bm{1} = 0, \\
%&\quad& \bm{\Omega}_{3,3} = 1, \\
%&\quad& \bm{\Omega} \succeq 0, 
%\end{eqnarray}
%The optimization problem $\mathcal{SDR}1$ can be efficiently solved to obtain the optimal solution $\bm{\Omega}^*$. If $\bm{\Omega}^*$ is of rank one, then $\bm{\Omega}^*$ is the optimal solution to \eqref{eq:opML} as well. Otherwise, $\bm{\Omega}^*$ is an approximation to the ML problem in \eqref{eq:opML}. 
%
%Gaussian randomization is a key method to find $\hat{\bm{\omega}}$ that is good enough and satisfy the constraints $\omega_n \in \{\pm 1 , \pm 3\}, \: n = 1, ..., 2N$. Gaussian randomization can be briefly summarized as follows. we generate $\check{\bm{\omega}}_{\ell}, \ell = 1, ..., L,$ where $L$ is the total number of generated RVs as $\check{\bm{\omega}}_{\ell} \sim (\bm{0}, \bm{\Omega}^*)$, then $\breve{\bm{\omega}}_{\ell} = {\rm{quantize}}\{\check{\bm{\omega}}_{\ell}\}$, where ${\rm{quantize}}(x)$ rounds $x$ to the nearest element in the set $\{\pm 1, \pm 3\}$. Finally, we find the solution as
%\begin{eqnarray}
%\ell^* & = & \arg \underset{\ell = 1, ..., L}{\min}  \Tr\{\bm{\Phi} \: \breve{\bm{\omega}} \: \breve{\bm{\omega}}^{\rm{T}}\}, \\
%\hat{\bm{\omega}} & = & \breve{\bm{\omega}}_{\ell^*}.
%\end{eqnarray}
%The constellation $\hat{\bm{a}}$ can be found from the first $2N$ elements in $\hat{\bm{\omega}}$.

In this section, we propose a STSDRSE technique to detect 16-QAM FTN signaling with reduced complexity. The proposed sequence estimation technique is more computationally efficient when compared to the proposed GASDRSE. As can be seen in $\mathcal{OP}_{\rm{GASDRSE}}$, the dimension of the decision matrix $\bm{\Omega}$ is $(4N + 1) \times (4N +1)$, where $N$ is the length of the complex data symbol vector. In this section, we reduce the dimension of the decision matrix, and hence,  decrease the computational complexity.

\subsection{Formulation of Quadratic Constraints}
We replace the generic high degree polynomial constraint  that models any high-order QAM, using concepts from the set theory, with a set of quadratic constraints suited to our particular case of interest in this paper, i.e., 16-QAM.
%Generic constraint formulation in our work \cite{bedeer2016low}
%In this paper, we reformulate the constraints in \cite{bedeer2016low} using concepts from set theory \cite{rosen1995discrete}.
%Another way to analyze the optimization problem in \eqref{eq:opML} is to handle the constraints in a different way as follows. 
Towards this goal, let us define the following sets 
\begin{eqnarray}
\mathcal{D}_1 &\coloneqq& (-\infty, -3), \nonumber \\
\mathcal{D}_2 &\coloneqq& (-3, -1), \nonumber \\
\mathcal{D}_3 &\coloneqq& (-1, 1), \nonumber \\
\mathcal{D}_4 &\coloneqq& (1, 3), \nonumber \\
\mathcal{D}_5 &\coloneqq& (3, \infty).
\end{eqnarray}
Then, the constraints in $\mathcal{OP}_{\rm{MLSE_c}}$ and $\mathcal{OP}_{\rm{MLSE_w}}$ can be expressed as \cite{ma2012semidefinite}
\begin{eqnarray}
\{\pm 1, \pm 3\} &=& \overline{\mathcal{D}_1 \cup \mathcal{D}_2 \cup \mathcal{D}_3 \cup \mathcal{D}_4 \cup \mathcal{D}_5}.
\end{eqnarray}
With the help of De Morgan's associative laws \cite{rosen1995discrete}, the constraints can be further rewritten as
\begin{eqnarray}
\{\pm 1, \pm 3\} &=& \overline{\mathcal{D}_1} \cap \overline{\mathcal{D}_2} \cap \overline{\mathcal{D}_3} \cap \overline{\mathcal{D}_4} \cap \overline{\mathcal{D}_5}, \nonumber \\
&=& ((\overline{\mathcal{D}_1} \cap \overline{\mathcal{D}_5}) \cap \overline{\mathcal{D}_3}) \cap \overline{\mathcal{D}_2} \cap \overline{\mathcal{D}_4} \nonumber \\
&=& ([-3, -1] \cup [1,3]) \cap \overline{\mathcal{D}_2} \cap \overline{\mathcal{D}_4}.
\end{eqnarray}
Accordingly, $[-3, -1] \cup [1,3]$, $\overline{\mathcal{D}_2}$, and $\overline{\mathcal{D}_2}$ can be respectively written as
\begin{eqnarray}
1 \leq a_n^2 \leq 9,  \label{eq:eq_1_n}\\
(a_n + 1)(a_n + 3) \geq 0,  \label{eq:eq_2_n}\\
(a_n - 1)(a_n - 3) \geq 0. \label{eq:eq_3_n}
\end{eqnarray}
To facilitate formulating the new SDR problem, let us reformulate $\mathcal{OP}_{\rm{MLSE_c}}$ and $\mathcal{OP}_{\rm{MLSE_w}}$ in a higher dimension by defining 
\begin{eqnarray}
\bm{\psi}^{\rm{T}} & = & [\bm{a}^{\rm{T}} \: 1], \nonumber \\
\bm{\Psi}_{ (2N + 1) \times (2N + 1)} & = & \bm{\psi} \: \bm{\psi}^{\rm{T}} =  \begin{bmatrix}
\bm{a} \bm{a}^{\rm{T}} & \bm{a}\\ 
\bm{a}^{\rm{T}}        & 1
\end{bmatrix}.
\end{eqnarray} 
The constraints in \eqref{eq:eq_1_n} - \eqref{eq:eq_3_n}   can be re-written in terms of $\bm{\Psi}$ as
\begin{eqnarray}
\bm{1}  \preceq  \diag\{\bm{\Psi}_{1,1}\} &\preceq& 9.\bm{1},  \label{eq:const_1_n1}\\
\diag\{\bm{\Psi}_{1,1}\} + 4 \: \bm{\Psi}_{1,2} + 3.\bm{1} &\succeq& 0, \label{eq:const_2_n1}\\ 
\diag\{\bm{\Psi}_{1,1}\} - 4 \: \bm{\Psi}_{1,2} + 3.\bm{1} &\succeq& 0, \label{eq:const_3_n1}\\
\bm{\Psi}_{2,2} &=& 1, \label{eq:const_41}
%\bm{\Psi} &\succeq& 0, \label{eq:const_5}\\
%\rank\{\bm{\Psi}\} &=& 1, \label{eq:const_6}
\end{eqnarray}
where  $\bm{\Psi}_{i,j}$, $i,j = 1, 2$ are the $(i,j)$th sub-blocks of $\bm{\Psi}$ of appropriate sizes, e.g., $\bm{\Psi}_{1,1} = \bm{a} \bm{a}^{\rm{T}}$ {(of size $2N \times 2N$)}, $\bm{\Psi}_{1,2} = \bm{a}$, $\bm{\Psi}_{2,1} = \bm{a}^{\rm{T}}$, and $\bm{\Psi}_{2,2} = 1$. The constraints in \eqref{eq:const_1_n1}, \eqref{eq:const_2_n1}, and \eqref{eq:const_3_n1} are equivalent to \eqref{eq:eq_1_n}, \eqref{eq:eq_2_n}, and \eqref{eq:eq_3_n}, respectively.

\subsection{Formulation of Objective Function}
--- \textit{General Pulse Shape: }
Since the matrix $\bm{G}$ is symmetric, the objective function of $\mathcal{OP}_{\rm{MLSE_c}}$  can be expressed in terms of $\bm{\Psi}$ as \cite{luo2010semidefinite, ma2012semidefinite}
\begin{eqnarray}
\bm{\psi}^{\rm{T}} \: \bm{\Theta}_{\textup{c}} \: \bm{\psi} = \Tr\{\bm{\Theta}_{\textup{c}} \: \bm{\psi} \: \bm{\psi}^{\rm{T}}\} = \Tr\{\bm{\Theta}_{\textup{c}} \: \bm{\Psi}\},
\end{eqnarray}
where 
\begin{eqnarray}
\bm{\Theta}_{{\textup{c}}, (2N + 1) \times (2N + 1)} = \begin{bmatrix}
\bm{G} & -\bm{y}_{\textup{c}}\\ 
- \bm{y}_{\textup{c}}^{\rm{T}} & \bm{z}^{\rm{T}} \bm{G} \bm{z}
\end{bmatrix}.
\end{eqnarray}

{
	--- \textit{rRC Pulse Shape: }
	For the case of rRC and for symmetric ISI matrix $\bm{V}$, the objective function of $\mathcal{OP}_{\rm{MLSE_w}}$ in \eqref{eq:opML_white} can be rewritten in terms of $\bm{\Psi}$ as {\cite{luo2010semidefinite, ma2012semidefinite}}
	\begin{eqnarray}
	\Tr\{\bm{\Theta}_{\textup{w}} \: \bm{\Psi}\},
	\end{eqnarray}
	where $\bm{\Theta}_{\textup{w}}$ is given by
	\begin{eqnarray}
	\bm{\Theta}_{\textup{w}} = \begin{bmatrix}
	\bm{V}^{\textup{T}} \bm{V} & -\bm{V}^{\textup{T}}\bm{y}_{\textup{w}}\\ 
	- \bm{y}_{\textup{w}}^{\rm{T}} \bm{V}             & \bm{y}_{\textup{w}}^{\rm{T}} \bm{y}_{\textup{w}}
	\end{bmatrix}.
	\end{eqnarray}
}

\subsection{SDR Optimization Problem and Proposed \textup{STSDRSE} Algorithm}

Finally, $\mathcal{OP}_{\rm{MLSE_c}}$ and $\mathcal{OP}_{\rm{MLSE_w}}$ can be casted as the following optimization problem
\begin{eqnarray}
\underset{\bm{\Psi}}{\min} &\quad&  \Tr\{\bm{\Theta} \: \bm{\Psi}\} \nonumber  \\
{\textup{subject to}} &\quad& \eqref{eq:const_1_n1}, \eqref{eq:const_2_n1}, \eqref{eq:const_3_n1},  \; {\rm{and}} \; \eqref{eq:const_41} \nonumber \\
&\quad& \bm{\Psi} \succeq 0, \label{eq:const_5}\\
&\quad& \rank\{\bm{\Psi}\} = 1, \label{eq:const_6}
\end{eqnarray}
where $\bm{\Theta}  \in \{\bm{\Theta}_{\textup{c}}, \bm{\Theta}_{\textup{w}}\}$ and   the constraints \eqref{eq:const_5} and \eqref{eq:const_6}   reflect that $\bm{\Psi}$ is  a  positive semidefinite and a rank-one matrix, respectively. It is clear that the above optimization problem is not convex due to the rank-one constraint in \eqref{eq:const_6}. By relaxing this constraint, we obtain an upper bound on its optimal solution as
\begin{eqnarray}\label{eq:SDRop2}
\mathcal{OP}_{\rm{STSDRSE}}:  \underset{\bm{\Psi}}{\min} &&  \Tr\{\bm{\Theta} \: \bm{\Psi}\} \nonumber  \\
{\textup{subject to}} && \eqref{eq:const_1_n1}, \eqref{eq:const_2_n1}, \eqref{eq:const_3_n1}, \eqref{eq:const_41}, \: {\rm{and}} \: \eqref{eq:const_5}, \nonumber  
\end{eqnarray}
which can be solved efficiently \cite{grant2010cvx} with polynomial time complexity.

Similar to the previous discussion of the proposed GASDRSE,   the optimal solution $\bm{\Psi}_{\textup{op}}$ of $\mathcal{OP}_{\rm{STSDRSE}}$ will not necessarily be a feasible solution of the original non-convex optimization problem; hence, we use Gaussian randomization to obtain an efficient feasible solution.
%An efficient method to obtain such a feasible solution is the Gaussian randomization. 
%The intuition behind Gaussian randomization is to solve a stochastic version of $\mathcal{OP}_{\rm{STSDRSE}}$, where the optimal solution $\psi^*$ is considered as the mean of a multivariate Gaussian random vector with zero mean and covariance matrix $\bm{\Psi}^*$.
We generate ${\bm{\zeta}} _{\ell}, \ell = 1, ..., L,$ as ${\bm{\zeta}} _{\ell} \sim (\bm{0}, \bm{\Psi}_{\textup{op}})$, then we quantized each random variable as $\breve{\bm{\psi}}_{\ell} = {\rm{quantize}}\{{\bm{\zeta}} _{\ell}\}$. Finally, we find the solution as
\begin{eqnarray}
\ell_{\textup{op}} & = & \arg \underset{\ell = 1, ..., L}{\min}  \Tr\{\bm{\Theta} \: \breve{\bm{\psi}}_{\ell} \: \breve{\bm{\psi}}_{\ell}^{\rm{T}}\}, \\
\hat{\bm{\psi}} & = & \breve{\bm{\psi}}_{\ell_{\textup{op}}}.
\end{eqnarray}
Finally, the estimated 16-QAM constellation vector $\hat{\bm{a}}$ is found from the first $2N$ elements in the vector $\hat{\bm{\psi}}$. 
%Finally, the estimated data symbols $\hat{\bm{a}}$ is found by selecting the first $2N$ elements in $\hat{\bm{\psi}}$. 

The proposed STSDRSE technique is formally expressed as follows 

%\textbf{\underline{Proposed SDR-based sequence estimation}:}
{\textit{Algorithm 2}: Proposed STSDRSE technique}
\begin{enumerate}
	\item \textbf{Input:} Pulse shape $g(t)$ {(ISI matrix $\bm{G}$)}, received samples $\bm{y}_{\textup{c}}$ and $\bm{y}_{\textup{w}}$, and number of randomization iterations $L$.
	\item Solve $\mathcal{OP}_{\rm{STSDRSE}}$  to find $\bm{\Psi}_{\textup{op}}$.
	\item Generate random variable ${\bm{\zeta}} _{\ell}$ as ${\bm{\zeta}} _{\ell} \sim (0, \bm{\Psi}_{\textup{op}})$, $\ell = 1, ..., L$.
	\item Find $\breve{\bm{\psi}}_{\ell} = {\rm{quantize}}\{{{\bm{\zeta}} _{\ell}\}}$.
	\item Find $\ell_{\textup{op}}  =  \arg \: \underset{\ell \:=\: 1, ..., L}{\min} \quad \Tr\{\bm{\Theta} \: \breve{\bm{\psi}}_{\ell} \: \breve{\bm{\psi}}_{\ell}^{\rm{T}}\}$.
	\item Set $\hat{\bm{\psi}} = \breve{\bm{\psi}}_{\ell_{\textup{op}}}$.
	\item \textbf{Output:} Estimated data symbols $\hat{\bm{a}}$ are the first $2 N$ elements of $\hat{\bm{\psi}}$.
\end{enumerate}


%shown in the top of the next page.
%\floatname{algorithm}{}
%\begin{algorithm}
%	\renewcommand{\thealgorithm}{}
%	\caption{\textbf{Proposed SDP-based Equalizer}}
%	\begin{algorithmic}[1]
%		%\small
%		\State \textbf{Input:} pulse shape $g(t)$, received samples $\bm{y}$, and number of randomization iterations $L$.
%		\State Solve $\mathcal{OP}_{\rm{STSDRSE}}$ in \eqref{eq:SDRop}  to find $\bm{\Psi}^*$.
%		\State Generate RV $\bm{\xi}_{\ell}$ as $\bm{\xi}_{\ell} \sim (0, \bm{\Psi}^*)$, $\ell = 1, ..., L$.
%		\State Find $\breve{\bm{\omega}}_{\ell} = {\rm{quantize}}\{{\bm{\xi}}_{\ell}\}$.
%		\State Find $\ell^*  =  \arg \: \underset{\ell \:=\: 1, ..., L}{\rm{minimize}} \quad \Tr\{\bm{\Theta} \: \breve{\bm{\psi}}_{\ell} \: \breve{\bm{\psi}}_{\ell}^{\rm{T}}\}$.
%		\State $\hat{\bm{\psi}} = \breve{\bm{\psi}}_{\ell^*}$.
%		\State \textbf{Output:} estimated data symbols $\hat{\bm{a}}$ as first $2 N$ elements of $\hat{\bm{\psi}}$.
%		%
%		%        \algstore{myalg}
%		%  \end{algorithmic}
%		%\end{algorithm}
%		%
%		%\floatname{algorithm}{}
%		%\begin{algorithm}
%		% % \ContinuedFloat
%		% \renewcommand{\thealgorithm}{}
%		%  \caption{\textbf{Proposed Algorithm} (continued)}
%		%  \begin{algorithmic}
%		%      \algrestore{myalg}
%		%     \small
%	\end{algorithmic}
%\end{algorithm}

%\subsection{Complexity Discussion}
%The computational complexity reduction of the proposed STSDRSE technique, when compared to the proposed GASDRSE, comes from the fact that the dimension of the unknown matrix $\bm{\Psi}$ is $(2 N + 1) \times (2 N + 1)$ which is smaller than its counterpart $\bm{\Omega}$ of $(4 N + 1) \times (4 N + 1)$ of the proposed GASDRSE. Accordingly, the computational complexity of the proposed STSDRSE technique is $\mathcal{O}((2N + 1)^{3.5} + (2N + 1)^{2} L)$.


{
\section{Comments On The Proposed \textup{GASDRSE} and \textup{STSDRSE} Techniques}\label{sec:comments}
\subsection{Complexity Discussion}

%Following \cite{luo2010semidefinite}, the worst case computation complexity  of the proposed GASDRSE technique is $\mathcal{O}((4N + 1)^{3.5} + (4N + 1)^{2} L)$. 
The worst case computational complexity of solving the relaxed $\mathcal{OP}_{\rm{GASDRSE}}$ is $\mathcal{O}((4N + 1)^{3.5}$ \cite{luo2010semidefinite}. Additionally, the complexity of generating and evaluating the objective function corresponding to the $L$ random samples of the Gaussian randomization is $\mathcal{O}((4N + 1)^{2} L$ \cite{luo2010semidefinite}. Hence, the total computational complexity of the proposed GASDRSE technique is $\mathcal{O}((4N + 1)^{3.5} + (4N + 1)^{2} L)$, which is polynomial in the received block length.

{
As mentioned earlier, the proposed GASDRSE technique can be extended to any high-order QAM FTN signaling,  with polynomial time computational complexity. For instance, for the case of 64-QAM FTN signaling, we need to use an additional auxiliary variable $c_n = b_n^2, n = 1, \hdots, 2N,$ in order to formulate the detection problem. In this case, the complexity of solving the relaxed $\mathcal{OP}_{\rm{GASDRSE}}$ is $\mathcal{O}((6N + 1)^{3.5}$, and the complexity of generating and evaluating the objective function corresponding to the $L$ random samples of the Gaussian randomization is $\mathcal{O}((6N + 1)^{2} L$. Hence, the overall  complexity of the proposed GASDRSE to detect 64-QAM FTN signaling will be in the order of $\mathcal{O}((6N + 1)^{3.5} + (6N + 1)^{2} L)$, which is still polynomial.} 

The computational complexity reduction of the proposed STSDRSE technique, when compared to the proposed GASDRSE, comes from the fact that the dimension of the unknown matrix $\bm{\Psi}$ is $(2 N + 1) \times (2 N + 1)$ which is smaller than its counterpart $\bm{\Omega}$ of $(4 N + 1) \times (4 N + 1)$ of the proposed GASDRSE. Accordingly, the computational complexity of the proposed STSDRSE technique is $\mathcal{O}((2N + 1)^{3.5} + (2N + 1)^{2} L)$.




	\subsection{Soft-Outputs}
The proposed GASDRSE and STSDRSE schemes produce hard-output, and in their current forms they may not be suitable to be used with channel coding. Fortunately, Gaussian randomization can be effectively used to reduce the complexity of evaluating the log-likelihood ratio (LLR) as follows. Inspired by the idea of the list sphere decoding in \cite{hochwald2003achieving}, the Gaussian randomization step can store a list of vectors that achieve the lowest values of the objective function (instead of storing only one vector that achieves the minimum objective value). This candidate list can then be used to approximate the LLR calculations. In other words, instead of searching the whole search space, Gaussian randomization can efficiently produce  candidate vectors that contribute more towards the calculation of the LLR equation. However, there is a possibility that some bit positions in the candidate list are empty. In this case, we can extend the candidate list to include all bit vectors with hamming distance of 1 of the bit vectors in the original candidate list as in \cite{love2005space}.
}

==> proposed.tex <==
\section{Dual Problem Solution \& Proposed Schemes} \label{sec:dual}

